Formulation Comparison for Timeline Construction using LLMs

Constructing a timeline requires identifying the chronological order of events in an article. In prior timeline construction datasets, temporal orders are typically annotated by either event-to-time anchoring or event-to-event pairwise ordering, both of which suffer from missing temporal information. To mitigate the issue, we develop a new evaluation dataset, TimeSET, consisting of single-document timelines with document-level order annotation. TimeSET features saliency-based event selection and partial ordering, which enable a practical annotation workload. Aiming to build better automatic timeline construction systems, we propose a novel evaluation framework to compare multiple task formulations with TimeSET by prompting open LLMs, i.e., Llama 2 and Flan-T5. Considering that identifying temporal orders of events is a core subtask in timeline construction, we further benchmark open LLMs on existing event temporal ordering datasets to gain a robust understanding of their capabilities. Our experiments show that (1) NLI formulation with Flan-T5 demonstrates a strong performance among others, while (2) timeline construction and event temporal ordering are still challenging tasks for few-shot LLMs. Our code and data are available at https://github.com/kimihiroh/timeset.

==> figures/concept_experiment.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{images/abstract2.png}
    \caption{An illustration of the difference between benchmarking and formulation comparison. Benchmarking (left) makes comparisons across models for each dataset (vertical arrow) but does not support comparisons across datasets (horizontal arrow). Our formulation comparison framework (right) supports comparisons across models and formulations (vertical, horizontal, and diagonal arrows).}
    \label{fig:concept}
\end{figure}

% think: add vertical line to left?

==> figures/summary.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{images/summary.png}
    \caption{Abstract illustration of traditional pairwise relation classification approach and autoregressive timeline generation approach.}
    \label{fig:summary}
\end{figure}

% probably better to replace the document icon with others
% or is it okay just to acknowledge the creator in appendix or something
% ap: i would use an actual example from the dataset, maybe a short paragraph as the document.
% km: replace the image with conceptual experiment illustration

==> tables/result_formulation_comparison.tex <==
\begin{table*}[!t]
\centering
\begin{adjustbox}{width=0.8\textwidth}
\begin{tabular}{l c c c c}
    \toprule
    &\multicolumn{4}{c}{Formulation}\\
    \cmidrule(lr){2-5}
    Model & NLI & Pairwise & MRC & Timeline \\
    \midrule
    Random & & & & \\
    Llama 2 (7B) & & & & \\
    Llama 2 Chat (7B) & & & & \\
    T5 (3B) & & & & \\
    Flan-T5 (3B) & & & & \\
    \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Result of formulation comparison}
\label{table:formulation_comparison_summary}
\end{table*}


==> tables/summary_formulations.tex <==
\begin{table}[!t]
\centering
\begin{adjustbox}{width=0.5\textwidth}
\begin{tabular}{l c c c}
    \toprule
    Formulation & Input & Output & \makecell{\#instance/doc \\ (\#event: $n$)} \\
    \midrule
    NLI & & & \\
    Pairwise & & & \\
    MRC & & & \\
    Timeline & & & \\
    \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Formulations}
\label{table:summary_formulations}
\end{table}

